Secure Information Flow Typing in LUSTRE

Synchronous reactive data flow is a paradigm that provides a high-level abstract programming model for embedded and cyber-physical systems, including the locally synchronous components of IoT systems. Security in such systems is severely compromised due to low-level programming, ill-defined interfaces and inattention to security classification of data. By incorporating a Denning-style lattice-based secure information flow framework into a synchronous reactive data flow language, we provide a framework in which correct-and-secure-by-construction implementations for such systems may be specified and derived. In particular, we propose an extension of the Lustre programming framework with a security type system. The novelty of our type system lies in a symbolic formulation of constraints over security type variables, in particular the treatment of node calls, which allows us to reason about secure flow with respect to any security class lattice. The main theorem is the soundness of our type system with respect to the co-inductive operational semantics of Lustre, which we prove by showing that well-typed programs exhibit non-interference. Rather than tackle the full language, we first prove the non-interference result for a well-behaved sub-language called "Normalised Lustre" (NLustre), for which our type system is far simpler. We then show that Bourke et al.'s semantics-preserving "normalisation" transformations from Lustre to NLustre are security-preserving as well. This preservation of security types by the normalisation transformations is a property akin to "subject reduction" but at the level of compiler transformations. The main result that well-security-typed Lustre programs are non-interfering follows from a reduction to our earlier result of non-interference for NLustre via the semantics-preservation (of Bourke et al.) and type preservation results.

==> LustreStreamSem.tex <==

\section{Lustre Stream Semantics}
\label{SEC:LustreStreamSem}

\begin{figure*}
    $$
    \begin{array}{c}
        \namedJdg{\semConst{c}{bs}{cs}}
        {\mstrSemExpPred{G,\Hst}{bs}{c}{[cs]}}{LScnst} ~~~
        %
        \namedJdg{\Hst(x)={\textcolor{BrickRed}{xs}}}
        {\mstrSemExpPred{G,\Hst}{bs}{x}{[xs]}}{LSvar} \\
        \\
        %
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
            {\liftunop{es}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\unop{e}}{[os]}}{LSunop} \\
        \\
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e_1}{[es_1]}}
            {\mstrSemExpPred{G,\Hst}{bs}{e_2}{[es_2]}}
            {\liftbinop{es_1}{es_2}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\binop{e_1}{e_2}}{[os]}}{LSbinop} \\
        \\
        \namedJdg{\predSet{\forall i ~\mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i}}
            {\hist{x}={\textcolor{BrickRed}{xs}}}
            {\forall i:~\mapwhenk{k}{xs}{\tupstrm{es}_i}{\tupstrm{os}_i}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\when{\vv{e_i}}{x=k}}{
        \flatten{\vv{\tupstrm{os}_i}}}}{LSwhn}\\
        \\
        \namedJdg{\dependSet{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
        {\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}}
        }
        {
           \forall j:~  \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j} 
            ~~~~
            \mapsemIte{es}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}
            }}
        {\mstrSemExpPred{G,\Hst}{bs}{\ite{e}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSite} \\
        \\
       \namedJdg{\dependSet{\predSet{\hist{x}=xs}{
       \forall i: ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}
       }}
            {\forall j: ~
            \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j}
            ~~~~
             \mapsemMerge{xs}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}}
            }
       {\mstrSemExpPred{G,\Hst}{bs}{\lmerge{x}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSmrg} \\
       \\
       \namedJdg{\predSet{\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{e0_i}{\tupstrm{e0s}_i}
      ~~~~ \forall j:~ 
       \mstrSemExpPred{G,\Hst}{bs}{e_j}{\tupstrm{es}_j}}
            { ~\mapsemLFby{(\flatten{\vv{\tupstrm{e0s}_i}})}{
            (\flatten{\vv{\tupstrm{es}_j}})}{\tupstrm{os}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\fby{\vv{e0_i}}{\vv{e_j}}}{\tupstrm{os}}}{LSfby} \\
   \\
        \namedJdg{\forall i \in [1,k] ~ \mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i} ~~~
        [\hist{x_1}, \ldots, \hist{x_n}] = 
        \flatten{\vv{\tupstrm{es}_i}}
        }
        {\mstrEqnPred{G}{\Hst}{bs}{\vv{x_j}=\vv{e_i}}}{LSeqn} \\
  \\
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{LSndef} \\
    \\
           \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{\vv{e_i}}{\tupstrm{xs}}}
            {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{f(\vv{e_i})}{\tupstrm{ys}}}{LSncall}
    \end{array}
    $$
    \caption{Stream semantics of \lustre}
    \label{FIG:LusStrSemNodeEqn}
\end{figure*}
% Name the Rules in a way consistent with the syntax
\begin{figure*}
    $$
    \begin{array}{c}
        \namedJdg{\semConst{c}{bs}{cs}}
        {\mstrSemExpPred{G,\Hst}{bs}{c}{[cs]}}{LScnst} ~~~
        %
        \namedJdg{\Hst(x)={\textcolor{BrickRed}{xs}}}
        {\mstrSemExpPred{G,\Hst}{bs}{x}{[xs]}}{LSvar} \\
        \\
        %
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
            {\liftunop{es}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\unop{e}}{[os]}}{LSunop} \\
        \\
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e_1}{[es_1]}}
            {\mstrSemExpPred{G,\Hst}{bs}{e_2}{[es_2]}}
            {\liftbinop{es_1}{es_2}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\binop{e_1}{e_2}}{[os]}}{LSbinop} \\
        \\
        \namedJdg{\predSet{\forall i ~\mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i}}
            {\hist{x}={\textcolor{BrickRed}{xs}}}
            {\forall i:~\mapwhenk{k}{xs}{\tupstrm{es}_i}{\tupstrm{os}_i}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\when{\vv{e_i}}{x=k}}{
        \flatten{\vv{\tupstrm{os}_i}}}}{LSwhn}\\
        \\
        \namedJdg{\dependSet{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
        {\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}}
        }
        {
           \forall j:~  \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j} 
            ~~~~
            \mapsemIte{es}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}
            }}
        {\mstrSemExpPred{G,\Hst}{bs}{\ite{e}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSite} \\
        \\
       \namedJdg{\dependSet{\predSet{\hist{x}=xs}{
       \forall i: ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}
       }}
            {\forall j: ~
            \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j}
            ~~~~
             \mapsemMerge{xs}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}}
            }
       {\mstrSemExpPred{G,\Hst}{bs}{\lmerge{x}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSmrg} \\
       \\
       \namedJdg{\predSet{\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{e0_i}{\tupstrm{e0s}_i}
      ~~~~ \forall j:~ 
       \mstrSemExpPred{G,\Hst}{bs}{e_j}{\tupstrm{es}_j}}
            { ~\mapsemLFby{(\flatten{\vv{\tupstrm{e0s}_i}})}{
            (\flatten{\vv{\tupstrm{es}_j}})}{\tupstrm{os}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\fby{\vv{e0_i}}{\vv{e_j}}}{\tupstrm{os}}}{LSfby} \\
   \\
        \namedJdg{\forall i \in [1,k] ~ \mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i} ~~~
        [\hist{x_1}, \ldots, \hist{x_n}] = 
        \flatten{\vv{\tupstrm{es}_i}}
        }
        {\mstrEqnPred{G}{\Hst}{bs}{\vv{x_j}=\vv{e_i}}}{LSeqn} \\
  \\
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{LSndef} \\
    \\
           \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{\vv{e_i}}{\tupstrm{xs}}}
            {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{f(\vv{e_i})}{\tupstrm{ys}}}{LSncall}
    \end{array}
    $$
    \caption{Stream semantics of \lustre}
    \label{FIG:LusStrSemNodeEqn}
\end{figure*}

The semantics of \lustre\ and \nlustre\  programs are \textit{synchronous}:
Each variable and expression defines a data stream which pulses with respect to a \textit{clock}.
A clock is a stream of booleans (CompCert/Coq's $\true$ and $\false$ in Velus).
A flow takes its $n^\tti{th}$ value on the $n^\tti{th}$ clock tick, \textit{i.e.},  some value, written $\stream{v}$, is present at instants when the clock value is \true, and none (written $\nullStream)$ when it is \false.
The \textit{temporal operators} \ttt{when}, \ttt{merge} and \ttt{fby} are used to express the complex clock-changing and clock-dependent behaviours of sampling, interpolation and delay respectively.


%Program behaviours in \lustre\ are completely determined by sequences of clocked occurrences of events.

Formally the stream semantics is defined using predicates over the program graph $G$, a (co-inductive) stream \textit{history} ($\Hst: \tti{Ident} \rightarrow \tti{value}~\tti{Stream}$) that associates value streams to variables, and a clock $bs$ \cite{Lustre2020,PYS-memocode2020,Bourke-jfla2021}.
Semantic operations on (lists of) streams are written in \textcolor{blue}{blue \textsf{sans serif}} typeface.
Streams are written in \textcolor{BrickRed}{red}, with lists of streams usually written in \textbf{\textcolor{BrickRed}{bold face}}.
All these stream operators, defined co-inductively,  enforce the clocking regime, ensuring  the presence of a value when the clock is \ckFont{true}, and absence when \ckFont{false}.

The predicate $\mstrSemExpPred{G,\Hst}{bs}{e}{\tupstrm{es}}$ relates an \textit{expression} $e$ to a \textit{list} of streams, written $\tupstrm{es}$.
A list consisting of only a single stream $\textcolor{BrickRed}{es}$ is explicitly denoted as $\textcolor{BrickRed}{[es]}$.
The semantics of \textit{equations} are expressed using the predicate 
$\mstrEqnPred{G}{\Hst}{bs}{\vv{eqn_i}}$, which requires \textit{consistency} between the assumed and defined stream histories in $\Hst$ for the program variables, as induced by the equations.
Finally, the semantics of \textit{nodes} is given as a stream history transformer predicate
$\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}.$

% Then reference the figure AND 
% explain the rules of the Figure.
Figure \ref{FIG:LusStrSemNodeEqn} presents the stream semantics for \lustre.
While rules for \textit{some} constructs have been variously presented \cite{SNLustre2017,Lustre2020,PYS-memocode2020,Bourke-jfla2021}, our presentation can be considered as a definitive consolidated specification of the operational semantics of \lustre, consistent with the V\'{e}lus compiler encoding \cite{Velus}.

Rule (LScnst) states that a constant $c$ denotes a constant stream of the value $\stream{c}$ pulsed according to given clock $bs$.  
This is effected by the semantic operator \ckFont{const}.
Rule (LSvar) associates a variable $x$ to the stream given by $\Hst(x)$. 
In rule (LSunop), \ckFont{$\hat{\diamond}$} denotes the operation $\diamond$ \textit{lifted} to apply instant-wise to the stream denoted by expression $e$.
Likewise in rule (LSbinop), the  binary operation $\oplus$ is applied paired point-wise to the streams denoted by the two sub-expressions (which should both pulse according to the same clock).
In all these rules, an expression is associated with a \textit{single} stream. 

The rule (LSwhn) describes \textit{sampling} whenever a variable $x$ takes the boolean value $k$, from the flows arising from a list of expressions $\vv{e_i}$,  returning a list of streams of such sampled values.
The predicate $\widehat{\ckFont{when}}$ \textit{maps} the predicate $\ckFont{when}$ to act on the corresponding components of \textit{lists} of streams, \textit{i.e.},  \[ 
\mapwhenk{k}{xs}{[es_1, \ldots, es_k]}{[os_1, \ldots, os_k]} 
~\textrm{abbreviates} ~ 
\bigwedge_{i \in [1,k]}~ \whenk{k}{xs}{es_i}{os_i}.
\]
(Similarly for the predicates
$\widehat{\ckFont{merge}}$, $\widehat{\ckFont{ite}}$, and $\widehat{\ckFont{fby}_L}$.  
The operation $\flatten{\_}$ flattens a list of lists (of possibly different lengths) into a single list. 
Flattening is required since expression $e_i$ may in general denote a \textit{list} of streams \textcolor{BrickRed}{$\tupstrm{es}_i$}.

The expression $\lmerge{x}{\vv{et}_i}{\vv{ef}_j}$ achieves (lists of) streams on a faster clock.
The semantics in rule (LSmrg) assume that for each pair of corresponding component streams from
$\flatten{\tupstrm{ets}_i}$ and
$\flatten{\tupstrm{efs}_j}$, a value is present in the first stream and absent in the second at those instances where $x$ has a true value $\stream{T}$, and complementarily, a value is present in the second stream and absent in the first when $x$ has a false value $\stream{F}$.
Both values must be absent when $x$’s value is absent.
These conditions are enforced by the auxiliary semantic operation \ckFont{merge}. 
In contrast, the conditional expression $\ite{e}{\vv{et}}{\vv{ef}}$
requires that all three argument streams $es$, and the corresponding components from $\flatten{\vv{\tupstrm{ets}_i}}$ and
$\flatten{\vv{\tupstrm{efs}_j}}$ pulse to the same clock.
Again, values are selected from the first or second component streams depending on whether the stream $es$ has the value $\stream{T}$ or $\stream{F}$ at a particular instant.
These conditions are enforced by the auxiliary semantic operation \ckFont{ite}. 
A delay operation is implemented by $\fby{e0}{e}$.
The rule (LSfby) is to be read as follows.
Let each expression $e0_i$ denote a list of streams
$\tupstrm{e0s_i}$, and each expression $e_j$ denote a list of streams $\tupstrm{es_j}$.
The output list of streams consists of streams whose first elements are taken from the each stream in $\flatten{\vv{\tupstrm{e0s}_i}}$ with the rest taken from the corresponding component of $\flatten{\vv{\tupstrm{es}_j}}$.
These are achieved using the semantic operation $\widehat{\ckFont{fby}_L}$.

The rule (LSeqn) for equations checks the consistency between the assumed meanings for the defined variables $x_j$ according to the history $\Hst$ with the corresponding components of the list of streams $\flatten{\vv{\tupstrm{es}_i}}$ to which a tuple of right-hand side expressions evaluates.

The rule (LSndef) presents the meaning given to a node definition $f$ as a stream list transformer. 
If history $\Hst$ assigns lists of streams to the input and output variables for a node a manner such that the semantics of the equations in the node are satisfied, then the semantics $\liftnode{f}$ transforms input stream list $\tupstrm{xs}$ to output stream list $\tupstrm{ys}$.
The operation \ckFont{base-of} finds an appropriate base clock with respect to which a given list of value streams pulse.
The rule (LSncall) uses the stream transformer semantics of $\liftnode{f}$ to the stream list $\tupstrm{xs}$ corresponding to the tuple of arguments $\vv{e_i}$, and returns the stream list $\tupstrm{ys}$.

\paragraph{Clocks and clock-annotated expressions.} \ 
We next present rules for clocks.
Further, we  assume that all (\nlustre) expressions in equations can be clock-annotated, and present the corresponding rules.

\begin{figure*}
$$
   \begin{array}{c}
        \namedJdg{}
        {\mstrSemCkPred{\Hst}{bs}{\ttt{base}}{bs}}{LSbase}  \\ \\
%        
        \namedJdg{
            \dependSet{\predSets{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\true}{bk}}}
            {\hist{x}=\cc{\stream{k}}{xs}}}
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\on{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\on{ck}{x}{k}}{\cc{\true}{bs'}}}{LSonT} \\
        
        
        \namedJdg{
            \dependSet{\predSets{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\false}{bk}}}
            {\hist{x}=\cc{\nullStream}{xs}}}
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\on{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\on{ck}{x}{k}}{\cc{\false}{bs'}}}{LSonA1} 
        \\
               \namedJdg{
            \dependSet{
             \predSet{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\true}{bk}}}
                {\hist{x}=\cc{\stream{k}}{xs}}
            }
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\onF{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\onF{ck}{x}{k}}{\cc{\false}{bs'}}}{LSonA2} \\ \\


        \namedJdg{\dependSet{\mstrSemExpPred{\Hst}{bs}{e}{[\ccnb{\nullStream}{es}]}}
        {\mstrSemCkPred{\Hst}{bs}{ck}{\ccnb{\false}{cs}}}}
    {\mstrSemExpPred{\Hst}{bs}{e::ck}{[\ccnb{\nullStream}{es}]}}{NSaeA} ~~
    
        \namedJdg{\dependSet{\mstrSemExpPred{\Hst}{bs}{e}{[\ccnb{\stream{v}}{es}]}}
            {\mstrSemCkPred{\Hst}{bs}{ck}{\ccnb{\true}{cs}}}}
        {\mstrSemExpPred{\Hst}{bs}{e::ck}{[\ccnb{\stream{v}}{es}]}}{NSae} 
    \end{array}
$$   
    \caption{Stream semantics of clocks and annotated expressions}
    \label{FIG:StrSemCk}
\end{figure*}

The predicate 
$\mstrSemCkPred{\Hst}{bs}{ck}{bs'}$ in \autoref{FIG:StrSemCk} defines the meaning of a \nlustre\ clock expression $ck$ with respect to a given history $\Hst$ and a clock $bs$ to be the resultant clock $bs'$.
% Note that a clock is a stream of booleans.  
The \ttt{on} construct lets us define 
coarser clocks derived from  a given clock --- whenever a variable $x$ has the desired value $k$ and the given clock is true. 
The rules (LSonT), (LSonA1), and (LSonA2) 
present the three cases: respectively when variable $x$ has the desired value $k$ and clock is true; the clock is false; and  the program variable $x$ has the complementary value and the clock is true.
The auxiliary operations \ckFont{tl} and \ckFont{htl},  give the tail of a stream, and the tails of streams for each variable according to a given history $\Hst$. 
Rules (NSaeA)-(NSae) describe the semantics of  clock-annotated expressions, where the output stream carries a value exactly when the clock is true.

\paragraph{Stream semantics for \nlustre.} \ \ 
The semantic relations for \nlustre\ are either identical to (as in constants, variables, unary and binary operations) or else the (simple) singleton cases of the rules given for \lustre\ (as in \ttt{merge}, \ttt{ite}, \ttt{when}).

The significant differences are in treatment of \ttt{fby}, and the occurrence of \ttt{fby} and node call only in the context of equations.

\begin{figure*}
   $$
    \begin{array}{c}
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\resClk{\Hst}{bs}}
        {\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{NSndef'} \\
    \\
%
        \namedJdg{\mstrSemExpPred{\Hst}{bs}{e::ck}{\hist{x}}}
        {\mstrEqnPred{G}{\Hst}{bs}{\eqn{x}{e}{ck}}}{NSeqn} 
\\ 
   \namedJdg{\predSet{\mstrSemExpPred{\Hst}{bs}{e::ck}{[vs]}}
            {\semFby{c}{vs}{\hist{x}}}}
        {\mstrEqnPred{G}{\Hst}{bs}{\eqn{x}{\fby{c}{e}}{ck}}}{NSfby'} \\
\\     
    \namedJdg{\predSet{\mstrSemExpPred{\Hst}{bs}{\vv{e}}{\tupstrm{vs}}}
    {\mstrSemCkPred{\Hst}{bs}{ck}{\baseOf{\tupstrm{vs}}}}
    {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{vs}}{\vv{\hist{x_i}}}}}
            {\mstrEqnPred{G}{\Hst}{bs}
        {\eqn{\vv{x}}{f(\vv{e})}{ck}  }}{NSncall'}
   
   \end{array}%  
    $$
    
    \caption{Stream semantics of \nlustre\ nodes and equations}
    \label{FIG:StrSemNodeEqn}
\end{figure*}

The (NSndef') rule only differs from (LSndef) in that 
post-transcription clock alignment, we have an additional requirement of $\Hst$ being in accordance with the base clock $bs$, enforced by \ckFont{respects-clock}.
The (NSdefn) rule for simple equations mentions the clock that annotates the defining expression, checking that it is consistent with the assumed history for the defined variable $x$.
The (NSdelay') rule for \ttt{fby} in an equational context uses the semantic operation \ckFont{fby}, which differs from $\ckFont{fby}_L$ in that it requires its first argument to be a constant rather than a stream.
Finally, the rule rule (NSncall') for node call, now in an equational context, is similar to (LSncall) except that it constrains the clock modulating the equation to be the base clock of the input flows.


